Unconditional Priors Matter! Improving Conditional Generation of Fine-Tuned Diffusion Models

Classifier-Free Guidance (CFG) is a fundamental technique in training conditional diffusion models. The common practice for CFG-based training is to use a single network to learn both conditional and unconditional noise prediction, with a small dropout rate for conditioning. However, we observe that the joint learning of unconditional noise with limited bandwidth in training results in poor priors for the unconditional case. More importantly, these poor unconditional noise predictions become a serious reason for degrading the quality of conditional generation. Inspired by the fact that most CFG-based conditional models are trained by fine-tuning a base model with better unconditional generation, we first show that simply replacing the unconditional noise in CFG with that predicted by the base model can significantly improve conditional generation. Furthermore, we show that a diffusion model other than the one the fine-tuned model was trained on can be used for unconditional noise replacement. We experimentally verify our claim with a range of CFG-based conditional models for both image and video generation, including Zero-1-to-3, Versatile Diffusion, DiT, DynamiCrafter, and InstructPix2Pix.

==> algorithms/cfg-tweedies.tex <==
\begin{algorithm}[t!]
\caption{CFG ($\mathbf{x}_{0|t}$-Formulation)}\label{alg:cfg-tweedies}
\begin{algorithmic}[1]
\State $\V{x}_T \sim \mathcal{N}(\mathbf{0},\V{I})$
\For{$t = T, \dots, 1$}
    \State \label{ln:conditional-tweedies}$\V{x}_{0 | t}^c = g(\V{x}_t, \epsilon_\theta (\V{x}_t, c)) \quad\text{\small{\texttt{// Conditional}}}$
    \State \label{ln:unconditional-tweedies}$\V{x}_{0 | t}^\emptyset = g(\V{x}_t, \epsilon_{\theta} (\V{x}_t, \emptyset))\quad\text{\small{\texttt{// Unconditional}}}$
    \State \label{ln:cfg-tweedies}$\V{x}_{0 | t}^{(\gamma)} = (1 - \gamma) \V{x}_{0 | t}^\emptyset + \gamma \V{x}_{0 | t}^c$
    \State \label{ln:renoise}$\V{x}_{t-1} = f(\V{x}_{0 | t}^{(\gamma)}, \epsilon_\theta^{(\gamma)}(\V{x}_t,c))$
\EndFor \\
\Return{$\mathbf{x}_0$}
\end{algorithmic}
\end{algorithm}

==> contents/004Method.tex <==
\vspace{-0.5\baselineskip}
\section{Rethinking CFG as Tweedie's Guidance}
\label{sec:cfg-tweedies-guidance}
\vspace{-0.25\baselineskip}

Let $\mathcal{M}$ and $\mathcal{M}^\star$ be the clean data manifolds corresponding to the true unconditional distribution $p(\V{x}_0)$ and fine-tuning data distribution $p^\star(\V{x}_0)$, respectively. Since the fine-tuning data manifold is a subset of the full data manifold, $\mathcal{M}^\star \subseteq \mathcal{M}$. Viewing the diffusion model as an EBM, CFG can be interpreted as generating samples from the gamma-powered distribution $p_\theta(\V{x}_0)^{(1-\gamma)} p_\theta(\V{x}_0 | c)^\gamma$ where $p_\theta$ approximates the true fine-tuning data distribution $p^\star$. Similarly, replacing the fine-tuned unconditional noise with the base model unconditional noise results in sampling from $p_\psi(\V{x}_0)^{(1-\gamma)} p_\theta(\V{x}_0 | c)^\gamma$.
The fine-tuning data distribution $p^\star(\V{x}_0)$ can be induced by restricting the domain of $p(\V{x}_0)$ to $\mathcal{M}^\star$: $p^\star(\V{x}_0) = p(\V{x}_0 | \V{x}_0 \in \mathcal{M}^\star)$. Using Bayes' theorem, 
{\small
\begin{align*}
    p^\star(\V{x}_0 = y) &= p(\V{x}_0 = y | \V{x}_0 \in \mathcal{M}^\star) \\
    &= \frac{p(\V{x}_0 \in \mathcal{M}^* | \V{x}_0 = y) p(\V{x}_0 = y)}{p(\V{x}_0 \in \mathcal{M}^\star)} \\
    &= p(\V{x}_0 = y) \frac{p(y \in \mathcal{M}^\star)}{p(\V{x}_0 \in \mathcal{M}^\star)}.
\end{align*}
}%
$p(\V{x}_0 \in \mathcal{M}^\star)$ is the ratio of the measures of $\mathcal{M}$ and $\mathcal{M}^\star$ which is a constant. For data $y \in \mathcal{M}^\star$, $p(y \in \mathcal{M}^\star) = 1$ therefore $p^\star(y)$ is equal to $p(y)$ (up to a constant). Then our method which samples from $p_\psi(\V{x}_0)^{(1-\gamma)} p_\theta(\V{x}_0 | c)^\gamma$ can be interpreted as sharpening the conditional modes of the distribution around the desired conditional modes as done in CFG.

==> figures/ip2p_comparison.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0.0}
    \begin{tabularx}{\linewidth}{Y | Y Y Y}
        \toprule
        Prompt & Input & Baseline & \textbf{w.r.} \\
        \midrule
        \raisebox{2.6em}{\makecell{\tiny \texttt{Add a}\\ \tiny\texttt{small sailboat}\\ \tiny\texttt{ visible in}\\ \tiny\texttt{ the distance.}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/00.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/01.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/02.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/03.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/04.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/05.jpg}} \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{\includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/editval/06.jpg}} \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{InstructPix2Pix Qualitative Results. Following the baseline, an Euler ancestral solver was used instead of DDIM.}
    \label{fig:ip2p-qual}
    \vspace{-0.5\baselineskip}
\end{figure}

\begin{figure}
    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0.0}
    \begin{tabularx}{\linewidth}{Y | Y Y Y}
        \toprule
        Prompt & Input & Baseline & \textbf{w.r.} \\
        \midrule
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/00.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/01.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/02.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/03.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/04.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/05.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/06.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{InstructPix2Pix Qualitative Results. Following the baseline, an Euler ancestral solver was used instead of DDIM.}
    \label{fig:ip2p-qual-2}
    \vspace{-0.5\baselineskip}
\end{figure}

\begin{figure}
    \centering
    \setlength{\tabcolsep}{0pt}
    \def\arraystretch{0.0}
    \begin{tabularx}{\linewidth}{Y | Y Y Y}
        \toprule
        Prompt & Input & Baseline & \textbf{w.r.} \\
        \midrule
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/07.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/08.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/09.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/10.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/11.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/12.jpg}
        } \\
        \raisebox{2.3em}{\makecell{\scriptsize \texttt{``PROMPT''}}} & \multicolumn{3}{c}{
            \includegraphics[width=0.75\linewidth]{figures/ip2p/tight-bbox/piebench/13.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{InstructPix2Pix Qualitative Results. Following the baseline, an Euler ancestral solver was used instead of DDIM.}
    \label{fig:ip2p-qual-3}
    \vspace{-0.5\baselineskip}
\end{figure}

==> figures/vd_comparison.tex <==
\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0em}
    \def\arraystretch{0.0}
    {\footnotesize
    \begin{tabularx}{P{0.25\textwidth}P{0.25\textwidth}P{0.25\textwidth}P{0.25\textwidth}}
        Input & CFG & UC & \textbf{Ours} \\
        \midrule
        \multicolumn{4}{c}{\includegraphics[width=\textwidth]{figures/versatile_diffusion/vd_row_1.jpg}} \\
    \end{tabularx}
    }
    \vspace{-0.5\baselineskip}
    \caption{Versatile Diffusion.}
    \label{fig:vd_comparison}
    \vspace{-0.5\baselineskip}
\end{figure*}

==> figures/vdiv_qualitatives.tex <==
\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\textwidth}{Y | Y Y Y | Y Y Y}
        \toprule
        \multirow{2}{*}{\makecell{Input\\Condition}} & \multicolumn{3}{c|}{CFG~\cite{ho2021classifier}} & \multicolumn{3}{c}{CFG++~\cite{chung2024cfg++}} \\
        & Baseline & +SD 1.4 & +SD 2.1 & Baseline & +SD 1.4 & +SD 2.1 \\  
        \midrule
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000061.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000005.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000006.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000012.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000013.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000017.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000029.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000030.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000031.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{Versatile Diffusion Qualitative Results}
    \label{fig:vdiv-qual}
    \vspace{-0.5\baselineskip}
\end{figure*}

\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{Y | Y Y Y | Y Y Y} 
        \toprule
        \multirow{2}{*}{\makecell{Input\\Image}} & \multicolumn{3}{c|}{CFG~\cite{ho2021classifier}} & \multicolumn{3}{c}{CFG++~\cite{chung2024cfg++}} \\
        & Baseline & +SD 1.4 & +SD 2.1 & Baseline & +SD 1.4 & +SD 2.1 \\  
        \midrule
        \multicolumn{7}{c}{
            \includegraphics[width=\textwidth]{figures/versatile-diffusion/000061.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\linewidth]{figures/versatile-diffusion/000062.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\linewidth]{figures/versatile-diffusion/000077.jpg}
        } \\
        \multicolumn{7}{c}{
            \includegraphics[width=\linewidth]{figures/versatile-diffusion/000104.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{Versatile Diffusion Qualitative Results}
    \label{fig:vdiv-qual-2}
    \vspace{-0.5\baselineskip}
\end{figure*}



==> figures/vdiv_selected_qualitatives.tex <==
\begin{figure*}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\textwidth}{Y | Y Y Y | Y Y Y}
        \toprule
        \multirow{3}{*}{\makecell{Input\\Image}} & \multicolumn{3}{c|}{CFG~\cite{ho2021classifier}} & \multicolumn{3}{c}{CFG++~\cite{chung2024cfg++}} \\
        & \makecell{VD\\\textbf{(Baseline)}} & \makecell{w/ SD1.4\\\textbf{(Ours)}} & \makecell{w/ SD2.1\\\textbf{(Ours)}} &
        \makecell{VD\\\textbf{(Baseline)}} & 
        \makecell{w/ SD1.4\\\textbf{(Ours)}} & 
        \makecell{w/ SD2.1\\\textbf{(Ours)}} \\
        \midrule 
        \multicolumn{7}{c}{\includegraphics[width=\textwidth]{figures/versatile-diffusion/selected-synthetic/540.jpg}} \\
        \multicolumn{7}{c}{\includegraphics[width=\textwidth]{figures/versatile-diffusion/selected-synthetic/381.jpg}} \\
        \multicolumn{7}{c}{\includegraphics[width=\textwidth]{figures/versatile-diffusion/selected-synthetic/464.jpg}} \\
        \bottomrule
    \end{tabularx}
    \vspace{-\baselineskip}
    \caption{\textbf{Image Variations with Versatile Diffusion~\cite{xu2023versatile}.} When using CFG or CFG++ with Versatile Diffusion, the outputs often suffer from style and detail degradation---excessive saturation (rows 1 and 3) or loss of key content (row 2). In contrast, our method, leveraging \texttt{SD1.4} and \texttt{SD2.1} as unconditional priors, achieves noticeable improvements in performance.}
    \label{fig:vdiv-selected-qualitatives}
    \vspace{-1.0\baselineskip}
\end{figure*}

==> figures/zero123_qualitatives.tex <==
\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{Y | Y | Y Y Y | Y Y Y}
        \toprule
        \multirow{3}{*}{\makecell{Input\\Image}} & \multirow{3}{*}{\makecell{Ground\\Truth}} & \multicolumn{3}{c|}{CFG~\cite{ho2021classifier}} & \multicolumn{3}{c}{CFG++~\cite{chung2024cfg++}} \\
        & & \multirow{2}{*}{\makecell{Zero-1-to-3\\\textbf{(Baseline)}}} & \multirow{2}{*}{\makecell{w/ SD1.4\\\textbf{(Ours)}}} & \multirow{2}{*}{\makecell{w/ SD2.1\\\textbf{(Ours)}}} & 
        \multirow{2}{*}{\makecell{Zero-1-to-3\\\textbf{(Baseline)}}} & \multirow{2}{*}{\makecell{w/ SD1.4\\\textbf{(Ours)}}} & \multirow{2}{*}{\makecell{w/ SD2.1\\\textbf{(Ours)}}} \\ \\
        \midrule
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/00.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/01.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/02.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/03.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/04.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/05.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/06.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/07.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/08.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/09.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{Zero 1-to-3 Qualitative Results}
    \label{fig:zero123-qual}
    \vspace{-0.5\baselineskip}
\end{figure*}

\begin{figure*}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{Y | Y | Y Y Y | Y Y Y}
        \toprule
        \multirow{3}{*}{\makecell{Input\\Image}} & \multirow{3}{*}{\makecell{Ground\\Truth}} & \multicolumn{3}{c|}{CFG~\cite{ho2021classifier}} & \multicolumn{3}{c}{CFG++~\cite{chung2024cfg++}} \\
        & & \multirow{2}{*}{\makecell{Zero-1-to-3\\\textbf{(Baseline)}}} & \multirow{2}{*}{\makecell{w/ SD1.4\\\textbf{(Ours)}}} & \multirow{2}{*}{\makecell{w/ SD2.1\\\textbf{(Ours)}}} 
        & \multirow{2}{*}{\makecell{Zero-1-to-3\\\textbf{(Baseline)}}} & \multirow{2}{*}{\makecell{w/ SD1.4\\\textbf{(Ours)}}} & \multirow{2}{*}{\makecell{w/ SD2.1\\\textbf{(Ours)}}} \\ \\
        \midrule
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/10.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/11.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/12.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/13.jpg}
        } \\
        \multicolumn{8}{c}{
        \includegraphics[width=\linewidth]{figures/zero123/tight-bbox/14.jpg}
        } \\
        \bottomrule
    \end{tabularx}
    \vspace{-0.5\baselineskip}
    \caption{Zero 1-to-3 Qualitative Results}
    \label{fig:zero123-qual-2}
    \vspace{-0.5\baselineskip}
\end{figure*}

==> latexmakerc.tex <==
$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';


==> tables/IP2P_CFG++_results.tex <==
\begin{table}
    \begin{minipage}{\linewidth}
    \centering
    \scriptsize
        % \begin{tabularx}{\linewidth}{c | Y | Y | Y | Y | Y}
        \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}m{0.175\textwidth} | >{\centering\arraybackslash}m{0.12\textwidth} | >{\centering\arraybackslash}m{0.12\textwidth} | >{\centering\arraybackslash}m{0.11\textwidth} | >{\centering\arraybackslash}m{0.09\textwidth} | > {\centering\arraybackslash}m{0.09\textwidth}}
        \toprule
         Method & CLIP-I $\uparrow$ & CLIP-T $\uparrow$ & \makecell{CLIP-D $\uparrow$} & \makecell{IR $\uparrow$} & PS $\uparrow$ \\
        \midrule
        IP2P (CFG++) & 0.780 & 0.202 & 0.116 & -2.025 & 0.142 \\
        w/ SD1.5 & \underline{0.919} & \underline{0.294} & \textbf{0.158} & \textbf{-0.406} & \textbf{0.490} \\
        w/ SD2.1 & \textbf{0.922} & \textbf{0.295} & \underline{0.157} & \underline{-0.436} & \textbf{0.490} \\
        \bottomrule
        \end{tabularx}
        \vspace{-0.5\baselineskip}
        \caption{\textbf{Image Editing with InstructPix2Pix (IP2P)~\cite{brooks2023instructpix2pix} using the CFG++ formulation.} We normalize text and image similarity scores: CLIP-I, CLIP-T, and CLIP-D. The PickScore (PS) baseline is IP2P \emph{CFG} which is shown in Tab.~\ref{tab:ip2p-results} \refinpaper{}.
        (\textbf{bold} represents the best, and \underline{underline} represents the second best method.)}
        \vspace{-\baselineskip}
    \label{tab:ip2p-results-cfg++}
    \end{minipage}
\end{table}

==> tables/SDIV_results.tex <==
\begin{table*}
\begin{minipage}{\linewidth}
\centering
\begin{tabularx}{\linewidth}{c || X | X | X | X}
% \toprule
% \multicolumn{4}{c}{\textbf{Versatile Diffusion Image Variations}}
\midrule
Method & FID-5k $\downarrow$ & $\text{FD}_{\text{DINOv2}}$-5k $\downarrow$ & CLIP-I $\uparrow$ & DINOv2 $\uparrow$ \\
\midrule
CFG                     & 41.035    & 635.777   & 0.903 & 0.824 \\
CFG w.r. (SD1.4)      & 38.368    & 609.618   & 0.910 & 0.831 \\
CFG w.r. (SD2.1)      &           &           &  & \\
\midrule
CFG++                   & 49.673    & 694.515   & 0.895 & 0.810 \\
CFG++ w.r. (SD1.4)    & 42.331    & 626.904   & 0.906 & 0.829 \\
CFG++ w.r. (SD2.1)    &           &           & &  \\
\bottomrule
\end{tabularx}
\caption{Stable Diffusion Image Variations}
\label{tab:sdiv-results}
\end{minipage}
\end{table*}

==> tables/VDIV_hyperparameters.tex <==
\begin{table}
    \begin{minipage}{\linewidth}
    \centering
    \scriptsize
        \begin{tabularx}{\linewidth}{Y | Y | Y Y}
        \toprule
        & \multirow{2}{*}{Method} & \multicolumn{2}{c}{FID-5k $\downarrow$} \\
        & & $\gamma=2.5$ & $\gamma=5.0$ \\
        \midrule
        \multirow{3}{*}{\textbf{CFG}} & VD & 39.088 & 42.333 \\
        & w/ SD1.4 & \textbf{35.430} & \textbf{35.596} \\
        & w/ SD2.1 & \underline{37.820} & \underline{38.444} \\
        \midrule
        & Method & $\gamma=0.5$ & $\gamma=0.8$ \\
        \midrule
        \multirow{3}{*}{\textbf{CFG++}} & VD & 44.038 & 46.740  \\
        & w/ SD1.4 & \textbf{36.102} & \textbf{37.105} \\
        & w/ SD2.1 & \underline{38.632} & \underline{38.625} \\
        \bottomrule
    \end{tabularx}
    \vspace{-1.0\baselineskip}
    \caption{\textbf{Image Variations with Versatile Diffusion.} Applying our sampling method achieves the best FID across various choices of $\gamma$. \textbf{Bold} represents the best, and \underline{underline} represents the second best method.}
    \label{tab:vdiv-hyperparameters-results}
    \vspace{-1.0\baselineskip}
    \end{minipage}
\end{table}

==> tables/Zero123_hyperparameter.tex <==
\begin{table*}
\begin{minipage}{\linewidth}
\centering
\scriptsize
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}m{0.10\textwidth} | Y | Y Y | Y Y | Y Y}
\toprule
 & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{LPIPS$\downarrow$} & \multicolumn{2}{c|}{PSNR$\uparrow$} & \multicolumn{2}{c}{SSIM$\uparrow$} \\
 & & $\gamma=3$ & $\gamma=4$ & $\gamma=3$ & $\gamma=4$ & $\gamma=3$ & $\gamma=4$ \\
\midrule
\multirow{3}{*}{\textbf{CFG}} & \scriptsize Zero-1-to-3 & 0.188 & 0.185 & 16.368 & 16.519 & 0.819 & 0.822 \\
& w/ \texttt{SD1.4} & \underline{0.170} & \underline{0.165} & \underline{17.327} & \underline{17.649} & \textbf{0.840} & \textbf{0.847} \\
& w/ \texttt{SD2.1} & \textbf{0.168} & \textbf{0.162} & \textbf{17.406} & \textbf{17.713} & \textbf{0.840} & \textbf{0.847} \\
\midrule
& Method & $\gamma=0.5$ & $\gamma=0.8$ & $\gamma=0.5$ & $\gamma=0.8$ & $\gamma=0.5$ & $\gamma=0.8$ \\
\midrule
\multirow{3}{*}{\textbf{CFG++}} & \scriptsize Zero1-to-3 & 0.185 & 0.182 & 16.621 & 16.706 & 0.822 & 0.824 \\
& w/ \texttt{SD1.4} & \underline{0.165} & \underline{0.162} & \underline{17.460} & \underline{17.562} & \underline{0.840} & \underline{0.841} \\
& w/ \texttt{SD2.1} & \textbf{0.158} & \textbf{0.155} & \textbf{17.814} & \textbf{17.903} & \textbf{0.848} & \textbf{0.849} \\
% w/ PixArt-$\alpha$ & 0.202 & 16.576 & 0.810 \\
\bottomrule
\end{tabularx}
\caption{\textbf{Novel View Synthesis with Zero-1-to-3.} Our method improves quality of novel view images on both CFG and CFG++ across various CFG scales (\textbf{bold} represents the best, and \underline{underline} represents the second best method).}
\label{tab:zero123-hyperparameters-results}
\vspace{-1.0\baselineskip}
\end{minipage}
\end{table*}


